Lagrange Duality and Compound Multi-Attention Transformer for Semi-Supervised Medical Image Segmentation

Medical image segmentation, a critical application of semantic segmentation in healthcare, has seen significant advancements through specialized computer vision techniques. While deep learning-based medical image segmentation is essential for assisting in medical diagnosis, the lack of diverse training data causes the long-tail problem. Moreover, most previous hybrid CNN-ViT architectures have limited ability to combine various attentions in different layers of the Convolutional Neural Network. To address these issues, we propose a Lagrange Duality Consistency (LDC) Loss, integrated with Boundary-Aware Contrastive Loss, as the overall training objective for semi-supervised learning to mitigate the long-tail problem. Additionally, we introduce CMAformer, a novel network that synergizes the strengths of ResUNet and Transformer. The cross-attention block in CMAformer effectively integrates spatial attention and channel attention for multi-scale feature fusion. Overall, our results indicate that CMAformer, combined with the feature fusion framework and the new consistency loss, demonstrates strong complementarity in semi-supervised learning ensembles. We achieve state-of-the-art results on multiple public medical image datasets. Example code are available at: \url{https://github.com/lzeeorno/Lagrange-Duality-and-CMAformer}.

==> figtex/fig1.tex <==
\begin{figure}[h]
\centerline{\includegraphics[width=\columnwidth]{figs/Overall Architecture.png}}
\caption{Adaptive Feature Fusion Semi-supervised Framework}
\label{fig1}
\end{figure}

==> figtex/fig4.tex <==
\begin{figure}[h]
\centerline{\includegraphics[width=\columnwidth]{figs/FeatureFusionBlock.png}}
\caption{Feature Fusion Bridge}
\label{fig4}
\end{figure}

==> figtex/fig5.tex <==
\begin{figure}[h]
\centerline{\includegraphics[width=1\columnwidth]{figs/ISICDM2019Result.png}}
\caption{ISICDM2019 Segmentation Result}
\label{fig5}
\end{figure}

==> tabletex/table1.tex <==
\begin{table}[h]
    \centering
    \caption{Comparison on size of state-of-the-art models}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{ccc}
        \toprule
        Model  & Params(M) & FLOPs(G) \\
        \midrule
        ResNet-101\cite{7resnet}    
            & 85.5 & 7.19      \\
        \hline
        % RegNetY-16G\cite{35RegNetY}  
        %     & 83.6 & 15.9      \\
        % \hline
        DeiT-B\cite{36DeiT}  
            & 86.6 & 17.6      \\
        \hline
        Swin-B\cite{37swin} 
            & 87.77 & 15.4     \\
        \hline
        % ConvNeXt-S\cite{38ConvNeXt}
        %     & 81.9 & 15.3     \\
        % \hline
        ResTv2-S\cite{resT2022v2}
            & 72.9 & 15.3     \\
        ResTv2-B
            & 87.6 & 6.34     \\
        \hline
        \textbf{ResUformer-T(Ours)}
            & \textbf{1.83} & \textbf{3.47}     \\
        \textbf{ResUformer-B(Ours)}
            & \textbf{67.65} & \textbf{6.63}     \\
        \textbf{ResUformer-L(Ours)}
            & \textbf{193.13} & \textbf{11.1}     \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:size}
\end{table}

==> tabletex/table3.tex <==
\begin{table}[!]
    \centering
    \caption{Comparison with State-of-the-Art models on the ISICDM2019 Dataset. The evaluation metric is DSC(\%). The best results are bolded while the second best are underlined. \ding{115} denotes uses larger inputs, whose size is 512x512. \ding{110} means small amount of extra training data. \ding{72} denotes uses self-design feature fusion preprocessing and data augmentation method. * denotes only use baseline or the baselines are implemented by ourselves. Thus, some comparison models without large-scale self-supervised pre-training guarantee a fair comparison.}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{c|c|c|c}
        \toprule
        Model  & Average & Bladder  & Tumor \\
               & DSC(\%) & DSC(\%)& DSC(\%) \\

        \midrule
        \midrule
        ViT\cite{34vit}+CUP\cite{15chen2021transunet}    
            & 88.6 & 91.88 & 85.32     \\
    
        R50-ViT\cite{34vit}+CUP\cite{15chen2021transunet}  
            & 87.88 & 92.05 & 85.49     \\

        ResUnet++\cite{53resunet++}*\ding{115}\ding{110}   
            & 87.11 & 89.9 & 84.32     \\
        
        ResT-V2-B\cite{resT2022v2}\ding{115}\ding{110}
            & 89.26 & 93.01 & 85.5     \\
            
        TransUNet\ding{110}\cite{15chen2021transunet} 
            & 91.7 & 94.98 & 88.42     \\

%        TransUNet\ding{115}\ding{110}\cite{15chen2021transunet}
%            & 92.81 & 96.04 & 89.58      \\
    
        SwinUNet\ding{110}\cite{21swinUnet2022}
            & 91.45 & 94.73 & 88.17    \\
            
        Swin UNETR*\ding{110}\cite{49swinUNETR}
            & 91.69 & 94.97 & 88.41     \\

        TransClaw U-Net\cite{18chang2021transclaw}
            & 91.49 & 94.75 & 88.22    \\

        LeViT-UNet-384s\cite{50levit}
            & 90.37 & 93.67 & 87.07     \\

        MISSFormer\ding{110}\cite{51missformer}
            & 91.62 & 94.89 & 88.35    \\

        CoTr*\cite{52cotr}
            & 90.92 & 94.19 & 87.65     \\

        UNETR*\cite{48unetr}
            & 91.55 & 94.83 & 88.26     \\

        nnFormer*\ding{110}\cite{47nnformer}
            & \underline{94.56}  & \underline{97.74} & 91.38     \\
        
        \hline
        \textbf{ResUformer-B(Ours)}*\ding{115}\ding{110}
            & 90.89 & 93.30 & 88.48     \\
        \textbf{ResUformer-B(Ours)}*\ding{115}\ding{110}\ding{72}
            & 93.59 & 95.63 & \underline{91.54}     \\
        \textbf{ResUformer-L-SSL(Ours)}*\ding{115}\ding{110}
            & 85.62 & 88.70 & 82.54      \\
        \textbf{ResUformer-L-SSL(Ours)}*\ding{115}\ding{110}\ding{72}
            & 87.71 & 90.47 & 84.95      \\
        \textbf{ResUformer-L(Ours)}*\ding{115}\ding{110}
            & 93.93 & 96.77 & 91.08         \\
        \textbf{ResUformer-L(Ours)}*\ding{115}\ding{110}\ding{72}
            & \textbf{96.06} & \textbf{98.57} & \textbf{93.56}     \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:isidm}
\end{table}

==> tabletex/table6.tex <==
\begin{table}[ht]
\centering
\caption{The experimental results of ablation study.}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Module} & \multicolumn{3}{c|}{Components} & \multicolumn{3}{c|}{RDD (512 $\times$ 512)} \\ \cline{2-7} 
                        & STD & EBO & CDGF & PSNR $\uparrow$ & SSIM $\uparrow$ & RMSE $\downarrow$ \\ \hline
\ding{55} & \ding{51} & \ding{51} & 26.92 & 0.91 & 12.1 \\ \hline
\ding{51} & \ding{55} & \ding{51} & 25.39 & 0.91 & 14.21 \\ \hline
\ding{51} & \ding{51} & \ding{55} & 27.87 & 0.92 & 10.84 \\ \hline
\ding{51} & \ding{51} & \ding{51} & \textbf{29.46} & \textbf{0.92} & \textbf{8.9} \\ \hline
\end{tabular}
\end{table}

==> temp.tex <==
% Consistency loss \cite{39consistencyloss} is a loss function used in deep learning to optimize models for producing consistent outputs under different input conditions. It is often employed to improve a model's robustness and ability to generate similar representations under different data augmentations. In self-training, consistency loss can be used to encourage the model to produce similar representations under different data augmentation methods, thereby improving the model's robustness to data augmentation.  The commonly used consistency loss function is mean squared error (MSE)\cite{40MSE}, but MSE is extremely sensitive to noise and unsuitable for complex data distributions. 

% Considering the semi-supervised feature fusion framework and medical image usage scenarios, the mean of BCEDice loss\cite{4unet} will be used as the consistency loss function of our semi-supervised feature fusion framework. The formula is:
% \begin{equation}
%     \sum_{n=1}^{N} [y_n \log(\hat{y}_n) + (1 - y_n) \log(1 - \hat{y}_n)] 
% \end{equation}
% The BCE-Dice loss combines two different loss functions to comprehensively consider pixel-level classification accuracy and segmentation similarity. However, for complex downstream tasks like multi-organ segmentation and small tumor segmentation, this loss function needs to be redesigned for convex optimization. 
% Therefore, we convert the Dice loss part into a Lagrangian dual problem\cite{42Lagrangianduality} with conditional constraints. However, Dice loss itself is not a convex function, so direct application of convex optimization theory is difficult. Auxiliary variables and additional constraints can be introduced to construct a related convex optimization problem. The Karush-Kuhn-Tucker (KKT) condition\cite{43KKT} can then be applied to construct a similar optimization framework.
% Converting the Dice loss to a convex optimization problem using Lagrangian duality and the KKT condition allows for more effective optimization of the BCE-Dice loss for complex medical image segmentation tasks. The feature fusion module also enables multi-scale feature learning to further improve segmentation performance.
% Taks LITS2017\cite{44lits2017} as an example, we have:
% % \begin{equation}
% %     \text{Dice1} = \frac{2 \times \sum_{i=1}^N P_{i_{1}} G_{i_{1}}}{\sum_{i=1}^N P_{i_{1}} + \sum_{i=1}^N G_{i_{1}}}
% % \end{equation}
% % \begin{equation}
% %     \text{Dice2} = \frac{2 \times \sum_{i=1}^N P_{i_{2}} G_{i_{2}}}{\sum_{i=1}^N P_{i_{2}} + \sum_{i=1}^N G_{i_{2}}}
% % \end{equation}

% \begin{equation}
%  \text{Dice}\left \{ j=1,2 \right \}  = \frac{2 \times \sum_{i=1}^N P_{i_{j}} G_{i_{j}}}{\sum_{i=1}^N P_{i_{j}} + \sum_{i=1}^N G_{i_{j}}}
% \end{equation}

% where $P_{ij}$ represents the model’s predicted probability that the $i^{th}$ pixel belongs to category (j). When (j=1) is liver label and (j=2) is tumor label. $G_{ij}$ is the corresponding ground truth label.
% To address the class imbalance problem, we propose a weighted Dice loss that assigns higher weights to tumors since they are generally more difficult to segment than the liver:
% \begin{equation}    
%     \begin{split}
%     New\ BCE\ Dice\ Loss = 
%     -\frac{1}{N} \sum_{i=1}^{N} [\alpha y_i\log(p_i) +\\
%     (\beta_1 \frac{y_{i_{1}} p_{i_{1}} }{y_{i_{1}} + p_{i_{1}}} + \beta_2 \frac{y_{i_{2}} p_{i_{2}} }{y_{i_{2}} + p_{i_{2}}} )]    
%     \end{split}
% \end{equation}



% Now, we have a convex optimization problem F(p) = argmin\{New BCE Dice Loss\}. Under this framework, we can introduce Lagrange multipliers to handle any possible constraints.
% \begin{enumerate}
%     \item Upper and lower bounds on the output value: 
    
%     ($ \mu_i^-  \leq F_i \leq \mu_i^+ $), for all (i).

%     \item Limitation on the sum of output values:

%     $\sum_{i=1}^N F_i =  \lambda$

%     \item The L2 norm limit of the model parameter vector ( W ) is:

%     $|w|_2^2 \leq \eta+C $, where ( C ) is a constant.

%     \item Non-negativity constraints:

%     $p_i = 1 - \zeta_i  \geq 0 $, for all (i).
% \end{enumerate}
% Among them,  $ \mu_i^-$, $ \mu_i^+$, $\lambda$, $\eta$ and $\zeta_i$ are the Lagrange multipliers introduced through constraints. Construct the Lagrangian function:
\begin{equation}    
    \begin{split}
    \mathcal{L}(p, w, \mu^+, \mu^-, \lambda, \eta, \zeta) =
    \sum_{i=1}^N (p_i - \mu_i^-) +  (\mu_i^+ - p_i) \\
    +\lambda (\sum_{i=1}^N p_i - S) 
    +\eta ( C - |w|_2^2) 
    +\sum_{i=1}^N \zeta_i (-p_i)    
    \end{split}
\end{equation}
% Solve the Lagrangian function by KKT conditions:
% \begin{enumerate}
%     \item[-] Stationarity: 
    
%     ($\frac{\partial \mathcal{L}}{\partial p_i} = 0$) and ($\frac{\partial \mathcal{L}}{\partial w} = 0$), for all i and w.

%     \item[-] Primal feasibility:

%     ($a \leq p_i \leq b$), ($|w|_2^2 \leq C $), ($ \mu_i^-  \leq F_i \leq \mu_i^+ $)

%     \item[-] Dual feasibility:

%     $[\mu_i^+ \geq 0,  \mu_i^- \geq 0,  \zeta_i \geq 0]$, for all i.

%     \item[-] Complementary slackness:

%     $[(\mu_i^+ - p_i) = 0, (p_i - \mu_i^-) = 0,  \zeta_i (-p_i) = 0]$, for all (i).
% \end{enumerate}
% In practice, this process is typically accomplished through gradient descent algorithms rather than analytical solutions. During training, we will use an SGD optimizer to iteratively update the model parameters and minimize the weighted Dice loss. After training for approximately 300 epochs on 5 different models, the optimal values of $\beta_1$ and $\beta_2$ in the weighted Dice loss function were found to be [0.314 ± 1e-5, 0.685 ± 1e-5] where i ranges from 1 to 9.
% Additionally, as long as the consistency loss based on the above KKT conditions is used, the segmentation results of small objects like tumors will be better than models that do not utilize this approach. 

==> theorem/theorem1.tex <==
\begin{algorithm}[tb]
    \caption{Semi-supervised Self-training Framework}
    \label{alg:algorithm}
    \textbf{Input}: labeled\_data, unlabeled\_data, epochs\\
    \textbf{Output}: Total Consistency Loss
    \begin{algorithmic}[1]
        \STATE Let $e=0$.
        \FOR{e in range of epochs}
            \STATE Define: ResUformer model $\xrightarrow{args}$ R
            \STATE Define: criterion = New\_BCE\_DICE($\alpha$,$\beta$)
            \FOR{CT, Mask in labeled\_data}
                \STATE Outputs = R(CT)
                \STATE $Loss_{supervised}$ = criterion(outputs, Mask)
                % \STATE $Loss_{supervised}$.backward()
            \ENDFOR
            \FOR{CT in unlabeled\_data}
                \STATE Outputs = R(CT)
                \STATE \_, Predicted\_Mask = Max(outputs,1)
                \STATE Pseudo\_Mask = Predicted\_Mask.detach()
                \STATE Pseudo\_out = R(CT)
                \STATE Consistency\_Loss = criterion(Outputs, Pseudo\_out)
                \STATE labeled\_data.append(CT, Pseudo\_Mask)
                \STATE $Loss_{unsupervised}$ = Consistency\_Loss
                % \STATE $Loss_{unsupervised}$.backward()
            \ENDFOR
        \ENDFOR
    \end{algorithmic}
\end{algorithm}

        % \IF {conditional}
        % \STATE Perform task A.
        % \ELSE
        % \STATE Perform task B.
        % \ENDIF
        % \STATE \textbf{return} solution
